Dual Operating Modes of In-Context Learning

In-context learning (ICL) exhibits dual operating modes: task learning, i.e., acquiring a new skill from in-context samples, and task retrieval, i.e., locating and activating a relevant pretrained skill. Recent theoretical work investigates various mathematical models to analyze ICL, but existing models explain only one operating mode at a time. We introduce a probabilistic model, with which one can explain the dual operating modes of ICL simultaneously. Focusing on in-context learning of linear functions, we extend existing models for pretraining data by introducing multiple task groups and task-dependent input distributions. We then analyze the behavior of the optimally pretrained model under the squared loss, i.e., the MMSE estimator of the label given in-context examples. Regarding pretraining task distribution as prior and in-context examples as the observation, we derive the closed-form expression of the task posterior distribution. With the closed-form expression, we obtain a quantitative understanding of the two operating modes of ICL. Furthermore, we shed light on an unexplained phenomenon observed in practice: under certain settings, the ICL risk initially increases and then decreases with more in-context examples. Our model offers a plausible explanation for this "early ascent" phenomenon: a limited number of in-context samples may lead to the retrieval of an incorrect skill, thereby increasing the risk, which will eventually diminish as task learning takes effect with more in-context samples. We also theoretically analyze ICL with biased labels, e.g., zero-shot ICL, where in-context examples are assigned random labels. Lastly, we validate our findings and predictions via experiments involving Transformers and large language models.

==> tex/App0TransformerSimulation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.90\textwidth]{figure/regular4.pdf}
    \vspace{-0.3cm}
    \caption{
    The figure shows the simulation of the Transformer under varied noise levels.
    $\sF$ indicates the prediction of Bayesian inference while $\hat{\F}$ indicates the prediction of the trained Transformer.
    One can observe that the lower the values of $\dm$ and $\dw$, \ie, the noise levels, the stronger the dip-and-rise phenomenon and the harder for the Transformer to approach the Bayesian inference.
    }
    \vspace{-0.5cm}
    \label{fig:regular4}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\textwidth]{figure/regularM.pdf}
    \caption{
    The figure shows the simulation of the Transformer under varied component densities.
    $\sF$ indicates the prediction of Bayesian inference while $\hat{\F}$ indicates the prediction of the trained Transformer.
    $M$ indicates the number of mixture components on the sphere with radius $1$, and $\dm=\dw=\frac{1}{16}$.
    It is observed that the higher the component density, the harder for the Transformer to approach the Bayesian inference.
    }
    \label{fig:regularM}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\textwidth]{figure/D_d.pdf}
    \caption{The figure shows the simulation of the Transformer under varied dimensions.
    $\sF$ indicates the prediction of Bayesian inference while $\hat{\F}$ indicates the prediction of the trained Transformer.
    $d$ indicates the dimension as well as the number of mixture components on the sphere with radius $1$, and $\dm=\dw=\frac{1}{16}$.
    It is observed that the higher the number of dimensions, the harder for the Transformer to approach the Bayesian inference.}
    \label{fig:D_d}
\end{figure}
\section{Additional Results of Transformer Simulation}
\label{app:transformer}
The Fig~\ref{fig:regular4}, Fig.~\ref{fig:regularM} and Fig.~\ref{fig:D_d} of experimental results of the Transformer model discussed in Sec.~\ref{sec:transformer} are shown here due to the page limitation.

In Fig~\ref{fig:regular4}, we consider the tetrahedron setting (see Apendix~\ref{sec:3d}) under varied task noises ($\dm=\dw \in \{1/256, 1/64, 1/16, 1/4, 1\}$).
The results show that the lower the variance, the stronger the dip-and-rise phenomenon in both Bayesian and Transformer inference, and it is also harder for the Transformer to capture the Bayesian prediction.
It also takes more training epochs for the Transformer to catch the Bayesian prediction when task noises are small.
In Fig~\ref{fig:regularM}, we consider settings of regular shapes (see Appendix~\ref{sec:3d}) with different numbers of vertices/components ($M\in\{4,6,8,12,20\}$).
In Fig~\ref{fig:D_d}, we consider settings with varied dimensions (see Appendix~\ref{sec:dd}, $d\in\{2,4,8,16,32\}$).
%Due to the page limitation, we put Fig~\ref{fig:regularM} and Fig~\ref{fig:D_d} into Appendix~\ref{app:transformer} as well the training setting.

\paragraph{Experiment Setting.} We conduct experiments based on the GPT2Model from the transformers package supported by Hugging Face. 
We use a 10-layer, 8-head Transformer decoder with 1024-dimensional feedforward layers, and the input dimension is set to $d$, equivalent to the dimension of $\vx$.
In each training epoch, we train the model with 10000 batches and each batch contains 256 samples.
We use AdamW~\cite{loshchilov2017decoupled} as the optimizer with weight decay as $0.00001$, and the learning rate is set to $0.00001$.

==> tex/App3CorollaryProof.tex <==
\section{Proof for Corollary~\ref{corollary:prediction}}
\label{sec:corollary}
This section shows the proof for Corollary~\ref{corollary:prediction}.\zq{I still remain the notation $\S_k+\vx_{k+1}$ since I'm not sure whether it should be changed.}
\begin{proof}
We prove by applying Assumption~\ref{asu:setting} to Eq.~\ref{equation:connection} and using Lemma~\ref{lemma:posterior}:
\begin{align}
&\sF(\S_k+\vx_{k+1}) \\
=& \displaystyle \mathop{\mathbb{E}}_{(\vm,\vw)\sim \Dpr} [
    \displaystyle \mathop{\mathbb{E}}_{y_{k+1}\mid\vx_{k+1}\sim \mathcal{D}_{y|\vx_{k+1}}(\vw)}   [y_{k+1}|\vw,\vx_{k+1}]|\S_k+\vx_{k+1}]
&(\text{Follow Eq.~\ref{equation:connection}})\\
=& \displaystyle \mathop{\mathbb{E}}_{(\vm,\vw)\sim \Dpr} [\langle \vw,\vx_{k+1} \rangle|\S_k+\vx_{k+1}]
&(\text{Apply Assumption~\ref{asu:setting}})\\
=& \sum_{\beta=1}^M \tpi_\beta \displaystyle\mathop{\mathbb{E}}_{(\vm,\vw)\sim \tT_\beta} [\langle \vw,\vx_{k+1} \rangle]
&(\text{Use Lemma~\ref{lemma:posterior}})\\
=& \sum_{\beta=1}^M \tpi_\beta \langle \tvw_\beta,\vx_{k+1} \rangle &(\text{Notice } \tT_\beta \text{is Gaussian})\\
=& \langle \sum_{\beta=1}^M \tpi_\beta\tvw_\beta,\vx_{k+1} \rangle
\end{align}
\end{proof}
